Efficient Processing of Deep Neural Networks: A Tutorial and Survey

Deep neural networks (DNNs) are currently widely used for many artificial intelligence (AI) applications including computer vision, speech recognition, and robotics. While DNNs deliver state-of-the-art accuracy on many AI tasks, it comes at the cost of high computational complexity. Accordingly, techniques that enable efficient processing of DNNs to improve energy efficiency and throughput without sacrificing application accuracy or increasing hardware cost are critical to the wide deployment of DNNs in AI systems. This article aims to provide a comprehensive tutorial and survey about the recent advances towards the goal of enabling efficient processing of DNNs. Specifically, it will provide an overview of DNNs, discuss various hardware platforms and architectures that support DNNs, and highlight key trends in reducing the computation cost of DNNs either solely via hardware design changes or via joint hardware design and DNN algorithm changes. It will also summarize various development resources that enable researchers and practitioners to quickly get started in this field, and highlight important benchmarking metrics and design considerations that should be used for evaluating the rapidly growing number of DNN hardware designs, optionally including algorithmic co-designs, being proposed in academia and industry. The reader will take away the following concepts from this article: understand the key design considerations for DNNs; be able to evaluate different DNN hardware implementations with benchmarks and comparison metrics; understand the trade-offs between various hardware architectures and platforms; be able to evaluate the utility of various DNN design techniques for efficient processing; and understand recent implementation trends and opportunities.

==> challenges.tex <==
\section{Challenges} 
The key metrics for DNN processing are accuracy, energy consumption, throughput, and cost.  The challenge is to address all these requirements concurrently.

As previously discussed, the accuracy of the DNN model should be measured for a well-defined task on a sufficiently large dataset (e.g., ImageNet).

%The computation of machine learning can often be higher than traditional signal processing tasks.  For instance, in the case of object detection, an image pyramid must be generated to detect objects of different sizes (or at different distances), which is 3$\times$ larger than a normal 2-D images~\cite{suleiman2014energy}.  Thus, machine learning can increase the dimensionality of the data that needs to be processed.

Energy consumption is often dominated by data movement as memory access consumes significantly more energy than computation~\cite{isscc2014-horowitz}.  This is particularly challenging for DNNs as the high dimensional representation and filters increase the amount of data generated, and the programmability needed to support different applications, tasks and networks means that the weights also need to be read and stored. In this paper, we will discuss various methods that reduce data movement to minimize energy consumption.  

The throughput is dictated by the amount of computation, which also increases with the dimensionality of the data. In this paper, we will discuss various transforms that can be applied to the data to reduce the number of required operations.

The cost is dictated by the amount of storage required on the chip. In this paper, we will discuss various methods to reduce storage costs such that the area of the chip is reduced, while maintaining low off-chip memory bandwidth.

% Finally, training requires a significant amount of labeled data (particularly for DNNs) as well as computation for multiple iterations of back-propagation to determine the value of the weights. There is on-going research on training in the cloud using CPUs, GPUs, FPGAs and ASICs. However, this is beyond the scope of this article.

Currently, state-of-the-art DNNs consume orders of magnitude higher energy than other forms of embedded processing (\eg, video compression)~\cite{iscas_2017}. We must exploit opportunities at multiple levels of hardware design to address all these challenges and close this energy gap.  Benchmarking Metrics for comparisons are summarized in Section~\ref{sec:benchmarking}.

